Color Image and Multispectral Image Denoising Using Block Diagonal Representation

Filtering images of more than one channel is challenging in terms of both efficiency and effectiveness. By grouping similar patches to utilize the self-similarity and sparse linear approximation of natural images, recent nonlocal and transform-domain methods have been widely used in color and multispectral image (MSI) denoising. Many related methods focus on the modeling of group level correlation to enhance sparsity, which often resorts to a recursive strategy with a large number of similar patches. The importance of the patch level representation is understated. In this paper, we mainly investigate the influence and potential of representation at patch level by considering a general formulation with block diagonal matrix. We further show that by training a proper global patch basis, along with a local principal component analysis transform in the grouping dimension, a simple transform-threshold-inverse method could produce very competitive results. Fast implementation is also developed to reduce computational complexity. Extensive experiments on both simulated and real datasets demonstrate its robustness, effectiveness and efficiency.

==> Submit_Arxiv_Zhaoming_Kong_Color_image/CMSt-SVD.tex <==
\begin{algorithm}
\caption{CMSt-SVD} %Ëã·¨µÄÃû×Ö
{\bf Input:} Noisy color image $\mathcal{A}$, $ps$, $SR$, $K$ and $N_{step}$.\\
{\bf Output:} Filtered image $\mathcal{A}_c$.\\
{\bf Step 1} (Global Training): The same as MSt-SVD.\\
{\bf Step 2} (Grouping): Given reference patch $\mathcal{P}_{ref}$, calculate its Euclidean distance with all patches in the Fourier domain using only the first slices via $||\hat{\mathcal{P}}_{ref}(:,:,1) - \hat{\mathcal{P}}_{i}(:,:,1)||_F$ to stack $K$ most similar patches in a group $\mathcal{G}$.\\
{\bf Step 3} (Collaborative filtering):\\
 \hspace*{0.2in}(1) Learn a factor matrix $\mathbf{U}_{group}$ in the last mode of third order tensor $\hat{\mathcal{G}}(:,:,1,:)$ in the Fourier domain via full PCA, and obtain the core tensor $\mathcal{C}$ via (\ref{compute_C_4D}).\\
 \hspace*{0.2in}(2) and (3) are the same as MSt-SVD.\\
{\bf Step 4} (Aggregation): The same as MSt-SVD.
\label{CMSt-SVD}
\end{algorithm}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_iid_cave.tex <==
\begin{figure*}[htbp]
\graphicspath{{MSI_image/i.i.d_gaussian/MC_new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.88in]{Origin_paint}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.88in]{noisy}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=0.88in]{4DHOSVD}}
\subfigure[TDL]{
\label{Fig4}
\includegraphics[width=0.88in]{TDL}}
\subfigure[BM4D]{
\label{Fig4}
\includegraphics[width=0.88in]{BM4D}}
\subfigure[LLRT]{
\label{Fig4}
\includegraphics[width=0.88in]{LLRT}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.88in]{global_tSVD}}


\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=1.06in]{Clean_crop_paint_new}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=1.06in]{4DHOSVD1_crop}}
\subfigure[TDL]{
\label{Fig4}
\includegraphics[width=1.06in]{TDL_crop}}
\subfigure[BM4D]{
\label{Fig4}
\includegraphics[width=1.06in]{BM4D_crop}}
\subfigure[LLRT]{
\label{Fig4}
\includegraphics[width=1.06in]{LLRT_crop}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.06in]{MSTSVD_crop}}


\caption{Visual evaluation of five competitive methods on CAVE dataset under i.i.d Gaussian noise with $\sigma = 100$.}

\label{fig_iid_cave}
\end{figure*}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_illus_CC15.tex <==
\begin{figure*}[htbp]
\graphicspath{{Illustration/Compare_dataset_CC15/Combine_new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=1.08in]{Clean_demo1_combine_paint}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo1_combine}}
%\subfigure[LSCD]{
%\label{Fig4}
%\includegraphics[width=1.16in]{LSCD_demo1_combine}}
\subfigure[FFD-Net]{
\label{Fig4}
\includegraphics[width=1.08in]{FFD-Net_demo1_combine}}
\subfigure[LLRT]{
\label{Fig5}
\includegraphics[width=1.08in]{LLRT_demo1_combine}}
\subfigure[GID]{
\label{Fig5}
\includegraphics[width=1.08in]{GID_demo1_combine}}\\

\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=1.08in]{TWSC_demo1_combine}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=1.08in]{MCWNNM_demo1_combine}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=1.08in]{4DHOSVD1_demo1_combine}}
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=1.08in]{CBM3D_demo1_combine}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{MS-TSVD_demo1_combine}}


\caption{Denoised images of compared methods on CC15. The camera is CANON D600 with ISO = 3200. Please zoom-in for better view.}

\label{Fig_illus_CC15_demo1}
\end{figure*}

\begin{figure*}[htbp]
\graphicspath{{Illustration/Compare_dataset_CC15/Combine_new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=1.08in]{Clean_demo2_combine_paint}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo2_combine}}
%\subfigure[LSCD]{
%\label{Fig4}
%\includegraphics[width=1.16in]{LSCD_demo2_combine}}
\subfigure[FFD-Net]{
\label{Fig4}
\includegraphics[width=1.08in]{FFD-Net_demo2_combine}}
\subfigure[LLRT]{
\label{Fig5}
\includegraphics[width=1.08in]{LLRT_demo2_combine}}
\subfigure[GID]{
\label{Fig5}
\includegraphics[width=1.08in]{GID_demo2_combine}}\\

\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=1.08in]{TWSC_demo2_combine}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=1.08in]{MCWNNM_demo2_combine}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=1.08in]{4DHOSVD1_demo2_combine}}
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=1.08in]{CBM3D_demo2_combine}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{MS-TSVD_demo2_combine}}


\caption{Denoised images of compared methods on CC15. The camera is NIKON D800 with ISO = 1600. Please zoom-in for better view.}

\label{Fig_illus_CC15_demo2}
\end{figure*}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_illus_CC60.tex <==
\begin{figure*}[htbp]
\graphicspath{{Illustration/Compare_dataset_CC60/Combine_new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=1.11in]{Clean_demo1_combine_paint}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.11in]{Noisy_demo1_combine}}
\subfigure[NI]{
\label{Fig4}
\includegraphics[width=1.11in]{NI_demo1_combine}}
\subfigure[LLRT]{
\label{Fig5}
\includegraphics[width=1.11in]{LLRT_new_demo1_combine}}
\subfigure[GID]{
\label{Fig5}
\includegraphics[width=1.11in]{GID_demo1_combine}}\\

\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=1.11in]{TWSC_demo1_combine}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=1.11in]{MCWNNM_demo1_combine}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=1.11in]{4DHOSVD1_demo1_combine}}
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=1.11in]{CBM3D_demo1_combine}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.11in]{MS-TSVD_demo1_combine}}


\caption{Denoised images of compared methods on CC60. The camera is NIKON D800 with ISO = 1600. Please zoom-in for better view.}

\label{Fig_illus_CC60}
\end{figure*}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_illus_Xu.tex <==
\begin{figure*}[htbp]
\graphicspath{{Illustration/Compare_dataset_Xu/Combine_new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=1.11in]{Clean_demo1_combine_paint}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.11in]{Noisy_demo1_combine}}
\subfigure[NI]{
\label{Fig4}
\includegraphics[width=1.11in]{NI_demo1_combine}}
\subfigure[LLRT]{
\label{Fig5}
\includegraphics[width=1.11in]{LLRT_demo1_combine}}
\subfigure[GID]{
\label{Fig5}
\includegraphics[width=1.11in]{GID_demo1_combine}}\\

\subfigure[TWSC]{
\label{Fig4}
\includegraphics[width=1.11in]{TWSC_demo1_combine}}
\subfigure[MCWNNM]{
\label{Fig4}
\includegraphics[width=1.11in]{MCWNNM_demo1_combine}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=1.11in]{4DHOSVD1_demo1_combine}}
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=1.11in]{CBM3D_demo1_combine}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.11in]{MST-SVD_demo1_combine}}


\caption{Dennoised images of compared methods on Xu's dataset. The camera is CANON 5D with ISO = 6400. Please zoom-in for better view.}

\label{Fig_illus_Xu}
\end{figure*}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_illus_bcirc_group.tex <==
\begin{figure}[htbp]
\graphicspath{{Illustration/Other/}}
\centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=3.38in]{bcirc_group}
  \caption{Block circulant representation of a group of similar patches.}

  \label{Fig_illus_bcirc_group}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_illus_paradigm.tex <==
\begin{figure}[htbp]
\graphicspath{{Illustration/Other/}}
\centering
\subfigure{
\label{Fig4}
\includegraphics[width=3.6in]{Flowchart}}

\caption{Flowchart of grouping-collaborative filtering-aggregation framework.}

\label{Fig_illus_paradigm}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_my_own.tex <==
\begin{figure}[htbp]
\graphicspath{{Illustration/Compare_my_own/new/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.79in]{mean_combine_paint}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.79in]{Noisy_combine}}
\subfigure[FFD-Net]{
\label{Fig4}
\includegraphics[width=0.79in]{FFD-Net_combine}}
\subfigure[CMSt-SVD]{
\label{Fig5}
\includegraphics[width=0.79in]{MSTSVD_combine}}


\caption{Denoised images of FFD-Net and CMSt-SVD on our dataset. The camera is HUAWEI Honor 6X with auto mode. Please zoom-in for better view.}

\label{Fig_my_own}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_non_iid_cave.tex <==
\begin{figure}[htbp]
\graphicspath{{MSI_image/non_i.i.d_gaussian/high_res/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=1.018in]{Origin_crop}}
\subfigure[4DHOSVD1]{
\label{Fig4}
\includegraphics[width=1.018in]{4DHOSVD_crop_paint}}
\subfigure[TDL]{
\label{Fig4}
\includegraphics[width=1.018in]{TDL_crop}}\\
\subfigure[BM4D]{
\label{Fig4}
\includegraphics[width=1.018in]{BM4D_crop}}
\subfigure[LLRT]{
\label{Fig4}
\includegraphics[width=1.018in]{LLRT_crop}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.018in]{global_tSVD_crop}}


\caption{Visual evaluation of compared methods under non i.i.d Gaussian noise.}

\label{fig_non_iid_cave}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_real_HDD.tex <==
\begin{figure}[htbp]
\graphicspath{{MSI_image/Real_HDD/Real_HDD_new/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.068in]{noisy_imgd3_paint}}
\subfigure[TDL]{
\label{Fig4}
\includegraphics[width=1.068in]{TDL_imgd3_new}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.068in]{MSTSVD_imgd3_new}}\\
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.068in]{noisy_imgd3_crop}}
\subfigure[TDL]{
\label{TDL_imgd3_crop_paint}
\includegraphics[width=1.068in]{TDL_imgd3_crop_paint}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.068in]{MSTSVD_imgd3_crop}}\\
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.068in]{noisy_imgd7_paint}}
\subfigure[TDL]{
\label{Fig4}
\includegraphics[width=1.068in]{TDL_imgd7_new}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.068in]{MSTSVD_imgd7_new}}\\
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.068in]{noisy_imgd7_crop}}
\subfigure[TDL]{
\label{TDL_imgd7_crop}
\includegraphics[width=1.068in]{TDL_imgd7_crop}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.068in]{MSTSVD_imgd7_crop}}


\caption{Visual evaluation of TDL and MSt-SVD on real HHD dataset. Please zoom in for better view.}

\label{fig_real_HDD}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_real_dnd.tex <==
\begin{figure}[htbp]
\graphicspath{{Illustration/DND/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.79in]{noisy_crop}}
\subfigure[Neat Image]{
\label{Fig4}
\includegraphics[width=0.79in]{test_filtered_NI_crop}}
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=0.79in]{test_filtered_CBM3D_crop}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.79in]{test_filtered_global_tSVD_crop}}


\caption{Visual comparison on real dnd dataset.}

\label{fig_real_dnd}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_real_urban.tex <==
\begin{figure}[htbp]
\graphicspath{{MSI_image/Real_urban/high_res/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.78in]{Noisy_103_crop}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.78in]{tSVD_103_crop}}
\subfigure[Nmog]{
\label{Fig4}
\includegraphics[width=0.78in]{Nmog_103_crop}}
\subfigure[twist MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.78in]{twist_tSVD_103_crop}}


\caption{Visual evaluation on band 103 in Urban data.}

\label{fig_real_urban1}
\end{figure}

\begin{figure}[htbp]
\graphicspath{{MSI_image/Real_urban/high_res/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=1.018in]{Noisy_1_crop}}
\subfigure[Nmog]{
\label{Fig4}
\includegraphics[width=1.018in]{Nmog_1_crop}}
\subfigure[twist MSt-SVD]{
\label{Fig4}
\includegraphics[width=1.018in]{twist_tSVD_1_crop}}


\caption{Visual evaluation on band 1 in Urban data.}

\label{fig_real_urban2}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_tau_tune.tex <==
\begin{figure}[htbp]
\graphicspath{{Discussion/}}

  \centering
  \includegraphics[width=2.6in]{tau_tune_new}


\caption{Average PSNR values of 4DHOSVD and MSt-SVD on the first 8 images of Kodak gallery when $\sigma = 30$ under different hard-threshold scale factor $\gamma$.}

\label{fig_tau_tune}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Fig_tau_tune_zoom_in.tex <==
\begin{figure}[htbp]
\graphicspath{{Discussion/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.68in]{origin_crop}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.68in]{noisy_crop}}
\subfigure[$\gamma = 1.2$]{
\label{Fig4}
\includegraphics[width=0.68in]{Brodatz_43_tSVD_tau_origin_crop}}
\subfigure[$\gamma = 1.4$]{
\label{Fig4}
\includegraphics[width=0.68in]{Brodatz_43_tSVD_tau_larger_crop}}


\caption{The influence of hard-threshold parameter on MSt-SVD when $\sigma = 60$.}

\label{fig_tau_tune_zoom_in}
\end{figure}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/MSt-SVD.tex <==
\begin{algorithm}[ht]
\caption{MSt-SVD} %Ëã·¨µÄÃû×Ö
{\bf Input:} Color or Multispectral image $\mathcal{A}$, patch size $ps$, local search window size $SR$, number of similar patches $K$, pixels between two adjacent reference patches $N_{step}$.\\
{\bf Output:} Filtered image $\mathcal{A}_c$.\\
{\bf Step 1} (Global Training): Train the global patch representation $\mathcal{U}_{row}$ and $\mathcal{U}_{column}$ with all reference patches using the nonlocal t-SVD in (\ref{nonlocal_tSVD}).\\
{\bf Step 2} (Grouping): Given reference patch $\mathcal{P}_{ref}$, calculate its Euclidean distance with all patches located in $SR$ via $||\mathcal{P}_{ref} - \mathcal{P}_{i}||_F$ to stack $K$ most similar patches in a group $\mathcal{G}$.\\
{\bf Step 3} (Collaborative filtering):\\
 \hspace*{0.2in}(1) Learn a factor matrix $\mathbf{U}_{group}$ in the 4-th mode of $\mathcal{G}$ via full PCA, and obtain the core tensor $\mathcal{C}$ via (\ref{compute_C_4D}).\\
 \hspace*{0.2in}(2) Apply the hard-threshold technique to $\mathcal{C}$, whose elements smaller than a certain threshold is set to zero.\\
 \hspace*{0.2in}(3) Obtain filtered group $\mathcal{G}_{filtered}$ via (\ref{compute_filtered_group}).\\
{\bf Step 4} (Aggregation): Averagely write back all image patches in $\mathcal{G}_d$ to their original locations.
\label{MSt-SVD}
\end{algorithm}


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_CAVE_origin.tex <==
% Table generated by Excel2LaTeX from sheet 'Origin'
%\begin{table*}[htbp]
%\ssmall
%  \centering
%  \caption{Quantitative results comparison under i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$ on CAVE dataset.}
%    \begin{tabular}{cccccccccccc}
%    \toprule
%    $\sigma$ & Index & Noisy & PARAFAC & LRTA  & LRMR  & 4DHOSVD1 & BM4D  & TDL   & ISTReg & LLRT  & MSt-SVD \\
%    \midrule
%    \multirow{4}[8]{*}{10} & PSNR  & 28.13  & 35.39  & 41.36  & 39.27  & 45.43  & 44.61  & 44.41  & 45.77  & 46.60  & 45.20  \\
%\cmidrule{2-12}          & SSIM  & 0.4371  & 0.8759  & 0.9499  & 0.9094  & 0.9811  & 0.9784  & 0.9797  & 0.9802  & 0.9868  & 0.9814  \\
%\cmidrule{2-12}          & ERGAS & 236.40  & 108.78  & 49.53  & 64.81  & 30.83  & 33.32  & 34.32  & 30.53  & 26.75  & 32.05  \\
%\cmidrule{2-12}          & SAM   & 0.7199  & 0.2363  & 0.1718  & 0.3343  & 0.1084  & 0.1289  & 0.1048  & 0.1086  & 0.0842  & 0.1064  \\
%    \midrule
%    \multirow{4}[8]{*}{30} & PSNR  & 18.59  & 33.65  & 36.06  & 31.36  & 39.78  & 38.80  & 39.07  & 40.51  & 41.49  & 40.23  \\
%\cmidrule{2-12}          & SSIM  & 0.1069  & 0.8294  & 0.8775  & 0.6451  & 0.9336  & 0.9283  & 0.9493  & 0.9488  & 0.9681  & 0.9530  \\
%\cmidrule{2-12}          & ERGAS & 676.01  & 125.13  & 90.50  & 157.65  & 59.12  & 65.23  & 63.18  & 53.05  & 48.50  & 56.26  \\
%\cmidrule{2-12}          & SAM   & 1.0085  & 0.3291  & 0.2446  & 0.6021  & 0.2272  & 0.2579  & 0.1493  & 0.1374  & 0.1221  & 0.1737  \\
%    \midrule
%    \multirow{4}[8]{*}{50} & PSNR  & 14.15  & 31.52  & 33.52  & 26.67  & 36.82  & 35.90  & 36.46  & 37.75  & 38.65  & 37.73  \\
%\cmidrule{2-12}          & SSIM  & 0.0475  & 0.7393  & 0.8201  & 0.4000  & 0.8722  & 0.8685  & 0.9171  & 0.9271  & 0.9482  & 0.9285  \\
%\cmidrule{2-12}          & ERGAS & 1126.70  & 154.19  & 121.15  & 264.28  & 83.36  & 91.19  & 85.24  & 70.16  & 67.56  & 75.03  \\
%\cmidrule{2-12}          & SAM   & 1.1461  & 0.4351  & 0.2897  & 0.7534  & 0.3385  & 0.3557  & 0.2008  & 0.1619  & 0.1551  & 0.2231  \\
%    \midrule
%    \multirow{4}[8]{*}{100} & PSNR  & 8.13  & 27.13  & 30.06  & 26.67  & 32.66  & 31.84  & 32.92  & 33.01  & 35.39  & 34.20  \\
%\cmidrule{2-12}          & SSIM  & 0.0136  & 0.4637  & 0.7138  & 0.1850  & 0.7307  & 0.7197  & 0.8284  & 0.8648  & 0.9154  & 0.8800  \\
%\cmidrule{2-12}          & ERGAS & 2253.40  & 250.68  & 180.03  & 469.26  & 134.34  & 144.91  & 128.15  & 120.77  & 99.37  & 115.24  \\
%\cmidrule{2-12}          & SAM   & 1.3074  & 0.6681  & 0.3649  & 0.9306  & 0.5599  & 0.5160  & 0.3132  & 0.2376  & 0.1962  & 0.3142  \\
%    \bottomrule
%    \end{tabular}%
%  \label{table_cave_origin1}%
%\end{table*}%


%% Table generated by Excel2LaTeX from sheet 'Origin'
%% Table generated by Excel2LaTeX from sheet 'Origin'
%\begin{table*}[htbp]
%\ssmall
%  \centering
%  \caption{Quantitative results comparison under i.i.d Gaussian noise $\sigma = \{150, 200\}$ on CAVE dataset.}
%    \begin{tabular}{cccccccccc}
%    \toprule
%    $\sigma$ & Index & Noisy & PARAFAC & LRTA  & 4DHOSVD1 & BM4D  & TDL   & LLRT  & MSt-SVD \\
%    \midrule
%    \multirow{4}[8]{*}{150} & PSNR  & 4.61  & 24.24  & 28.15  & 30.27  & 29.36  & 30.76  & 33.41  & 32.08  \\
%\cmidrule{2-10}          & SSIM  & 0.0059  & 0.2800  & 0.6315  & 0.6474  & 0.5947  & 0.7366  & 0.8859  & 0.8401  \\
%\cmidrule{2-10}          & ERGAS & 3380.10  & 348.28  & 223.95  & 174.66  & 192.16  & 163.43  & 124.62  & 147.97  \\
%\cmidrule{2-10}          & SAM   & 1.3816  & 0.8088  & 0.4237  & 0.6961  & 0.6189  & 0.4100  & 0.2288  & 0.3788  \\
%    \midrule
%    \multirow{4}[8]{*}{200} & PSNR  & 2.11  & 22.12  & 26.70  & 28.54  & 27.54  & 29.14  & 32.01  & 30.59  \\
%\cmidrule{2-10}          & SSIM  & 0.0031  & 0.1814  & 0.5571  & 0.5911  & 0.4955  & 0.6490  & 0.8592  & 0.8040  \\
%\cmidrule{2-10}          & ERGAS & 4506.70  & 445.16  & 264.91  & 210.65  & 236.94  & 196.81  & 145.45  & 174.67  \\
%\cmidrule{2-10}          & SAM   & 1.4241  & 0.8933  & 0.4668  & 0.7773  & 0.6927  & 0.4974  & 0.2559  & 0.4284  \\
%    \bottomrule
%    \end{tabular}%
%  \label{table_cave_origin2}%
%\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Origin'
\begin{table*}[htbp]
\ssmall
  \centering
  \caption{Quantitative results comparison under i.i.d Gaussian noise $\sigma = \{10, 30, 50, 100\}$ on CAVE dataset.}
    \begin{tabular}{ccccccccccccccccc}
    \toprule
    \multirow{2}[4]{*}{Methods} & \multicolumn{4}{c}{$\sigma = 10$} & \multicolumn{4}{c}{$\sigma = 30$} & \multicolumn{4}{c}{$\sigma = 50$} & \multicolumn{4}{c}{$\sigma = 100$} \\
\cmidrule{2-17}          & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM   & PSNR  & SSIM  & ERGAS & SAM \\
    \midrule
    Noisy & 28.13  & 0.4371 & 236.40  & 0.7199 & 18.59  & 0.1069 & 676.01  & 1.0085 & 14.15 & 0.0475  & 1126.7 & 1.1461 & 8.13  & 0.0136  & 2253.4 & 1.3074  \\
    \midrule
    PARAFAC & 35.39  & 0.8759 & 108.78  & 0.2363 & 33.65  & 0.8294 & 125.13  & 0.3291 & 31.52 & 0.7393  & 154.19 & 0.4351 & 27.13  & 0.4637  & 250.68 & 0.6681  \\
    \midrule
    LRTA  & 41.36  & 0.9499 & 49.53  & 0.1718 & 36.06  & 0.8775 & 90.50  & 0.2446 & 33.52 & 0.8201  & 121.15 & 0.2897 & 30.06  & 0.7138  & 180.03 & 0.3649  \\
    \midrule
    LRMR  & 39.27  & 0.9094 & 64.81  & 0.3343 & 31.36  & 0.6451 & 157.65  & 0.6021 & 26.67 & 0.4000  & 264.28 & 0.7534 & 26.67  & 0.1850  & 469.26 & 0.9306  \\
    \midrule
    4DHOSVD1 & 45.43  & 0.9811 & 30.83  & 0.1084 & 39.78  & 0.9336 & 59.12  & 0.2272 & 36.82 & 0.8722  & 83.36 & 0.3385 & 32.66  & 0.7307  & 134.34 & 0.5599  \\
    \midrule
    BM4D  & 44.61  & 0.9784 & 33.32  & 0.1289 & 38.80  & 0.9283 & 65.23  & 0.2579 & 35.98  & 0.8685  & 91.19 & 0.3557 & 31.84  & 0.7197  & 144.91 & 0.5160  \\
    \midrule
    TDL   & 44.41  & 0.9797 & 34.32  & 0.1048 & 39.07  & 0.9493 & 63.18  & 0.1493 & 36.46 & 0.9171  & 85.24 & 0.2008 & 32.92  & 0.8284  & 128.15 & 0.3132  \\
    \midrule
    ISTReg & 45.77  & 0.9802 & 30.53  & 0.1086 & 40.51  & 0.9488 & 53.05  & 0.1374 & 37.75 & 0.9271  & 70.16 & 0.1619 & 33.01  & 0.8648  & 120.77 & 0.2376  \\
    \midrule
    LLRT  & 46.60  & 0.9868 & 26.75  & 0.0842 & 41.49  & 0.9681 & 48.50  & 0.1221 & 38.65 & 0.9482  & 67.56 & 0.1551 & 35.39  & 0.9154  & 99.37 & 0.1962  \\
    \midrule
    MSt-SVD & 45.20  & 0.9814 & 32.05  & 0.1064 & 40.23  & 0.9530 & 56.26  & 0.1737 & 37.73 & 0.9285  & 75.03 & 0.2231 & 34.20  & 0.8800  & 115.24 & 0.3142  \\
    \bottomrule
    \end{tabular}%
  \label{table_cave_origin1}%
\end{table*}%




==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_CAVE_unbalance.tex <==

\begin{table}[htbp]
\ssmall
  \centering
  \caption{Quantitative results comparison under non i.i.d Gaussian noise with input noise level $\sigma = 36$ for all compared methods on CAVE dataset.}
    \begin{tabular}{cccccccc}
    \toprule
    Index & PARAFAC & LRTA & 4DHOSVD1 & BM4D & TDL & LLRT & MSt-SVD \\
    \midrule
    PSNR  & 32.7 & 33.0 & 38.1  & 36.6 & 32.3 & 38.3 & 39.3  \\
    \midrule
    SSIM  & 0.79 & 0.74 & 0.91  & 0.86 & 0.74 & 0.92 & 0.94  \\
    \midrule
    ERGAS & 137.9 & 132.6 & 71.9 & 89.7 & 140.9 & 70.8 & 62.4  \\
    \midrule
    SAM   & 0.40 & 0.45 & 0.33 & 0.40 & 0.48 & 0.21 & 0.19  \\
    \midrule
    Time (m) & 4.8 & 0.6 & 5.5 & 10.1 & 1.2 & 48.8 & 6.2 \\
    \bottomrule
    \end{tabular}%
  \label{table_cave_unbalance}%
\end{table}%




==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_CC60_Xu.tex <==
% Table generated by Excel2LaTeX from sheet 'dataset2_3'
\begin{table*}[htbp]
\scriptsize
  \centering
  \caption{Average PSNR and SSIM values of compared methods on CC60 and Xu-100 datasets. The best results are bolded.}
    \begin{tabular}{cccccccccccc}
    \toprule
    Dataset & Index & LLRT  & WTR1  & FFD-Net & GID   & TWSC  & MCWNNM & 4DHOSVD1 & CBM3D & CBM3D\_best & CMSt-SVD \\
    \midrule
    \multirow{2}[4]{*}{CC60} & PSNR  & 38.51  & 39.69  & \textbf{39.73 } & 38.41  & 39.66  & 39.03  & 39.15  & 39.40  & 39.68  & \textbf{39.75 } \\
\cmidrule{2-12}          & SSIM  & 0.9636  & 0.9764  & 0.9770  & 0.9633  & 0.9759  & 0.9698  & 0.9729  & 0.9740  & \textbf{0.9775 } & 0.9756  \\
    \midrule
    \multirow{2}[4]{*}{Xu} & PSNR  & 38.51 & 38.56 & 38.56  & 38.37 & 38.62 & 38.51 & 38.51 & 38.69 & \textbf{38.81} & \textbf{38.82} \\
\cmidrule{2-12}          & SSIM  & 0.9707 & 0.9669 & 0.9658  & 0.9675 & 0.9674 & 0.9671 & 0.9673 & 0.9694 & \textbf{0.9712} & 0.9694 \\
    \bottomrule
    \end{tabular}%
  \label{Table_CC60_Xu}%
\end{table*}%


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_Real_ccnoise.tex <==
% Table generated by Excel2LaTeX from sheet 'Result'
\begin{table*}[htbp]
\ssmall
  \centering
  \caption{PSNR results and average computational time (s) of different methods on 15 cropped real noisy images used in \cite{nam2016holistic}.}
    \begin{tabular}{cccccccccccccccccc}
    \toprule
    Methods & \multicolumn{3}{c}{Canon 5D ISO = 3200} & \multicolumn{3}{c}{Canon D600 ISO = 3200} & \multicolumn{3}{c}{Nikon D800 ISO = 1600} & \multicolumn{3}{c}{Nikon D800 ISO = 3200} & \multicolumn{3}{c}{Nikon D800 ISO = 6400} & Average & Time (s) \\
    \midrule
    LSCD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 9.68  \\
    \midrule
    LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & 1198 \\
    \midrule
    MLP   & 39.00  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & N/A \\
    \midrule
    DnCNN & 37.26  & 34.13  & 34.09  & 33.62  & 34.48  & 35.41  & 35.79  & 36.08  & 35.48  & 34.08  & 33.70  & 33.31  & 29.83  & 30.55  & 30.09  & 33.86  & N/A \\
    \midrule
    MCWNNM & 41.20  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & \textbf{37.72 } & 318.29  \\
    \midrule
    CBM3D & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & \textbf{37.69 } & 6.98  \\
    \midrule
    4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 120.18  \\
    \midrule
    MSt-SVD & 40.33  & 37.25  & 36.83  & 35.16  & 36.71  & 40.29  & 38.97  & 41.49  & 39.24  & 39.61  & 37.43  & 39.93  & 34.34  & 33.82  & 33.96  & \textbf{37.69 } & 110.06  \\
    \bottomrule
    \end{tabular}%
  \label{table_real_ccnoise}%
\end{table*}%




==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_cc15.tex <==

% Table generated by Excel2LaTeX from sheet 'dataset 1'
\begin{table*}[htbp]
  \centering
  \ssmall
  \caption{PSNR results and average computational time (s) of different methods on CC15 dataset. The three best results are bolded.}
    \begin{tabular}{cccccccccccccccccc}
    \toprule
    Methods & \multicolumn{3}{c}{Canon 5D ISO = 3200} & \multicolumn{3}{c}{Canon D600 ISO = 3200} & \multicolumn{3}{c}{Nikon D800 ISO = 1600} & \multicolumn{3}{c}{Nikon D800 ISO = 3200} & \multicolumn{3}{c}{Nikon D800 ISO = 6400} & Average & Time (s) \\
    \midrule
    LSCD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 9.68  \\
    \midrule
    LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & $>1000$ \\
    \midrule
    WTR1  & 41.09  & 36.92  & 36.25  & 34.68  & 36.48  & 40.52  & 38.26  & 41.40  & 38.61  & 39.98  & 37.70  & 41.36  & 35.16  & 34.22  & 34.43  & 37.81  & $>2000$ \\
    \midrule
    TNRD  & 39.51  & 36.47  & 36.45  & 34.79  & 36.37  & 39.49  & 38.11  & 40.52  & 38.17  & 37.69  & 35.90  & 38.21  & 32.81  & 32.33  & 32.29  & 36.61  & N/A \\
    \midrule
    MLP   & 39.00  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & N/A \\
    \midrule
    DnCNN & 37.26  & 34.13  & 34.09  & 33.62  & 34.48  & 35.41  & 35.79  & 36.08  & 35.48  & 34.08  & 33.70  & 33.31  & 29.83  & 30.55  & 30.09  & 33.86  & N/A \\
    \midrule
    GID   & 40.82  & 37.19  & 36.92  & 35.32  & 36.62  & 38.68  & 38.88  & 40.66  & 39.20  & 37.92  & 36.62  & 37.64  & 33.01  & 32.93  & 32.96  & 37.02  & 55.60  \\
    \midrule
    WCMNNM & 41.20  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & 37.72  & 318.29  \\
    \midrule
    FFD-Net & 39.40  & 37.02  & 36.53  & 34.97  & 36.73  & 41.02  & 38.66  & 41.53  & 38.80  & 40.15  & 37.61  & 41.18  & 34.13  & 33.66  & 33.69  & 37.68  & 28.98  \\
    \midrule
    TWSC  & 40.55  & 35.92  & 35.15  & 35.36  & 37.09  & 41.13  & 39.36  & 41.91  & 38.81  & 40.27  & 37.22  & 42.09  & 35.53  & 34.15  & 33.93  & \textbf{37.90 } & 480.80  \\
    \midrule
    CBM3D & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & 37.69  & 6.98  \\
    \midrule
    CBM3D\_best & 40.96  & 37.31  & 37.15  & 35.38  & 36.81  & 40.45  & 39.25  & 41.65  & 39.59  & 39.86  & 37.54  & 40.38  & 34.85  & 33.92  & 34.16  & \textbf{37.95 } & 6.98  \\
    \midrule
    4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 120.18  \\
    \midrule
    MSt-SVD & 40.33  & 37.25  & 36.83  & 35.16  & 36.71  & 40.29  & 38.97  & 41.49  & 39.24  & 39.61  & 37.43  & 39.93  & 34.34  & 33.82  & 33.96  & 37.69  & 110.06  \\
    \midrule
    CMSt-SVD & 40.79  & 37.37  & 37.01  & 35.29  & 36.95  & 40.93  & 39.21  & 41.98  & 39.54  & 39.98  & 37.65  & 40.05  & 34.50  & 33.93  & 34.01  & \textbf{37.95 } & 98.88  \\
    \bottomrule
    \end{tabular}%
  \label{Table_cc15}
\end{table*}%


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_dataset_description.tex <==
% Table generated by Excel2LaTeX from sheet 'Sub'
% Table generated by Excel2LaTeX from sheet 'Sub'
\begin{table}[htbp]
  \centering
  \caption{Brief description of three real-world color image datasets.}
    \begin{tabular}{cccc}
    \toprule
    Dataset & Type  & \# of Images & Image Size \\
    \midrule
    CC15 \cite{nam2016holistic}  & Real-World & 15    & $512 \times 512$ \\
    \midrule
    CC60  \cite{xu2018external} & Real-World & 60    & $500 \times 500$ \\
    \midrule
    Xu-100    \cite{DatasetXu} & Real-World & 100   & $512 \times 512$ \\
    \midrule
    Ours    \cite{KongData} & Real-World & 249   & $1024 \times 1024$ \\
    \bottomrule
    \end{tabular}%
  \label{Table_dataset_description}%
\end{table}%



==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_my_own.tex <==
% Table generated by Excel2LaTeX from sheet 'dataset 4'
\begin{table*}[htbp]
\ssmall
  \centering
  \caption{Average PSNR and SSIM values of compared methods on our dataset. The best results are bolded. The input noise level of compared methods are tuned to produce their best average results of every camera.}
    \begin{tabular}{cccccccccccc}
    \toprule
    Camera & \# of Images & Index & LLRT  & FFD-Net & GID   & TWSC  & MCWNNM & 4DHOSVD1 & CBM3D & CBM3D\_best & CMSt-SVD \\
    \midrule
    \multirow{2}[4]{*}{HUAWEI HONOR 6X} & \multirow{2}[4]{*}{30} & PSNR  & 39.54 & 40.05  & 39.52  & 39.71  & 39.46 & 39.82 & 39.97 & \textbf{40.48} & 40.08 \\
\cmidrule{3-12}          &       & SSIM  & 0.9669 & 0.9669  & 0.9653 & 0.9651 & 0.9610  & 0.9658  & 0.9669  & \textbf{0.9740 } & 0.9674  \\
    \midrule
    \multirow{2}[4]{*}{IPHONE 5S} & \multirow{2}[4]{*}{36} & PSNR  & 40.02 & 40.60  & 40.12  & 40.27  & 39.87 & 40.68 & 40.77 & \textbf{41.25} & 40.84 \\
\cmidrule{3-12}          &       & SSIM  & 0.9676 & 0.9645  & 0.9642 & 0.9617 & 0.9567  & 0.9664  & 0.9668  & \textbf{0.9758 } & 0.9668  \\
    \midrule
    \multirow{2}[4]{*}{IPHONE 6S} & \multirow{2}[4]{*}{67} & PSNR  & 39.72 & 40.49  & 40.16  & 40.12  & 40.18 & 40.36 & 40.55 & \textbf{41.16} & 40.53 \\
\cmidrule{3-12}          &       & SSIM  & 0.9663 & 0.9707  & 0.9670  & 0.9619  & 0.9628  & 0.9671  & 0.9693  & \textbf{0.9783 } & 0.9674  \\
    \midrule
    \multirow{2}[4]{*}{CANON 100D} & \multirow{2}[4]{*}{55} & PSNR  & 41.84 & 41.67  & 40.86 & 41.65 & 41.47 & 41.41 & 41.69 & \textbf{42.08} & 41.99 \\
\cmidrule{3-12}          &       & SSIM  & 0.9784 & 0.9768  & 0.9743  & 0.9767  & 0.9774  & 0.9771  & 0.9780  & \textbf{0.9808 } & 0.9794  \\
    \midrule
    \multirow{2}[4]{*}{CANON 600D} & \multirow{2}[4]{*}{25} & PSNR  & 42.53 & 42.55  & 41.60  & 42.52  & 42.07 & 42.14 & 42.54 & \textbf{42.89} & 42.75 \\
\cmidrule{3-12}          &       & SSIM  & 0.9816 & 0.9824  & 0.9790  & 0.9824  & 0.9795  & 0.9810  & 0.9836  & \textbf{0.9851 } & 0.9840  \\
    \midrule
    \multirow{2}[4]{*}{SONY A6500} & \multirow{2}[4]{*}{36} & PSNR  & 45.71 & 45.71  & 44.94  & 45.48  & 45.37 & 45.56 & 45.70  & 45.81 & \textbf{45.89} \\
\cmidrule{3-12}          &       & SSIM  & 0.9899 & 0.9901  & 0.9887  & 0.9896  & 0.9894  & 0.9901  & 0.9902  & \textbf{0.9904 } & 0.9903  \\
    \bottomrule
    \end{tabular}%
  \label{Table_my_own}%
\end{table*}%


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_para_choice.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\ssmall
  \centering
  \caption{Choice of parameters for 4DHOSVD and MSt-SVD on color image and multispectral image (MSI) experiments.}
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}[4]{*}{Parameter} & \multicolumn{2}{c}{4DHOSVD} & \multicolumn{2}{c}{MSt-SVD} \\
\cmidrule{2-5}          & Color Image & MSI   & Color Image & MSI \\
    \midrule
    $ps$    & 8    & 8    & 8     & 8  \\
    \midrule
    $K$     & 30    & 30    & 30    & 30 \\
    \midrule
    $SR$    & 20    & 16    & 20    & 16 \\
    \midrule
    $N_{step}$ & 4     & 4     & 4     & 4 \\
    \midrule
    $\gamma$ & 0.8     & 1     & 1.1 ($\sigma<30$), 1.2 ($\sigma>30$)    & 4 \\
    \bottomrule
    \end{tabular}%
  \label{table_para_choice}%
\end{table}%


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_sigma_chosen.tex <==
% Table generated by Excel2LaTeX from sheet 'sigma'
\begin{table}[htbp]
  \centering
  \caption{Input noise level of Gaussian denoisers for CC15, CC60 and Xu-100 datasets.}
    \begin{tabular}{ccccc}
    \toprule
    Method & LSCD  & WTR1  & FFD-Net & LLRT \\
    \midrule
    $\sigma$ & 10    & 15    & 15    & 20 \\
    \midrule
    Method & 4DHOSVD1 & CBM3D & MSt-SVD & CMSt-SVD \\
    \midrule
    $\sigma$ & 30    & 20    & 30    & 25 \\
    \bottomrule
    \end{tabular}%
  \label{Table_sigma_chosen}%
\end{table}%


==> Submit_Arxiv_Zhaoming_Kong_Color_image/Table_technique_briefing.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\ssmall
  \centering
    \caption{Techniques and priors adopted by different methods based on the grouping-collaborative filtering-aggregation framework. LR: Low Rank; SC: Sparse Coding; HT: Hard-thresholding; WF: Wiener Filter \cite{Dabov2007Image}}
    \begin{tabular}{ccccccccc}
    \toprule
    Method & LLRT \cite{chang2017hyper}  & WTR1 \cite{Li2018Weighted}   & TWSC \cite{TrilateralXu}  & NCSR \cite{Dong2013Sparse} & CBM3D & Proposed\\
    \midrule
    Techique & LR   &  LR     & SC    & SC & HT+WF & HT\\
    \bottomrule
    \end{tabular}%
  \label{Table_technique_briefing}%
\end{table}%


==> Table_Real_ccnoise.tex <==
% Table generated by Excel2LaTeX from sheet 'Result'
\begin{table*}[htbp]
\ssmall
  \centering
  \caption{PSNR results and average computational time (s) of different methods on 15 cropped real noisy images used in \cite{nam2016holistic}.}
    \begin{tabular}{cccccccccccccccccc}
    \toprule
    Methods & \multicolumn{3}{c}{Canon 5D ISO = 3200} & \multicolumn{3}{c}{Canon D600 ISO = 3200} & \multicolumn{3}{c}{Nikon D800 ISO = 1600} & \multicolumn{3}{c}{Nikon D800 ISO = 3200} & \multicolumn{3}{c}{Nikon D800 ISO = 6400} & Average & Time (s) \\
    \midrule
    LSCD  & 37.86  & 36.21  & 35.52  & 34.65  & 36.26  & 38.24  & 37.90  & 38.88  & 38.32  & 37.45  & 36.49  & 37.73  & 32.33  & 32.55  & 32.62  & 36.20  & 9.68  \\
    \midrule
    LLRT  & 39.23  & 36.31  & 35.93  & 34.74  & 36.83  & 40.58  & 37.39  & 40.27  & 37.78  & 39.79  & 37.34  & 41.03  & 35.09  & 34.05  & 34.11  & 37.36  & 1198 \\
    \midrule
    MLP   & 39.00  & 36.34  & 36.33  & 34.70  & 36.20  & 39.33  & 37.95  & 40.23  & 37.94  & 37.55  & 35.91  & 38.15  & 32.69  & 32.33  & 32.29  & 36.46  & N/A \\
    \midrule
    DnCNN & 37.26  & 34.13  & 34.09  & 33.62  & 34.48  & 35.41  & 35.79  & 36.08  & 35.48  & 34.08  & 33.70  & 33.31  & 29.83  & 30.55  & 30.09  & 33.86  & N/A \\
    \midrule
    MCWNNM & 41.20  & 37.25  & 36.48  & 35.54  & 37.03  & 39.56  & 39.26  & 41.45  & 39.54  & 38.94  & 37.40  & 39.42  & 34.85  & 33.97  & 33.97  & \textbf{37.72 } & 318.29  \\
    \midrule
    CBM3D & 40.77  & 37.31  & 36.98  & 35.21  & 36.76  & 40.13  & 39.02  & 41.65  & 39.40  & 39.59  & 37.49  & 39.47  & 34.13  & 33.73  & 33.85  & \textbf{37.69 } & 6.98  \\
    \midrule
    4DHOSVD1 & 40.22  & 36.97  & 36.55  & 35.02  & 36.60  & 39.78  & 38.85  & 41.35  & 39.11  & 39.24  & 37.28  & 39.47  & 34.40  & 33.81  & 34.01  & 37.51  & 120.18  \\
    \midrule
    MSt-SVD & 40.33  & 37.25  & 36.83  & 35.16  & 36.71  & 40.29  & 38.97  & 41.49  & 39.24  & 39.61  & 37.43  & 39.93  & 34.34  & 33.82  & 33.96  & \textbf{37.69 } & 110.06  \\
    \bottomrule
    \end{tabular}%
  \label{table_real_ccnoise}%
\end{table*}%



